Scalable and Energy-Efficient Millimeter Massive MIMO Architectures: Reflect-Array and Transmit-Array Antennas

Hybrid analog-digital architectures are considered as promising candidates for implementing millimeter wave (mmWave) massive multiple-input multiple-output (MIMO) systems since they enable a considerable reduction of the required number of costly radio frequency (RF) chains by moving some of the signal processing operations into the analog domain. However, the analog feed network, comprising RF dividers, combiners, phase shifters, and line connections, of hybrid MIMO architectures is not scalable due to its prohibitively high power consumption for large numbers of transmit antennas. Motivated by this limitation, in this paper, we study novel massive MIMO architectures, namely reflect-array (RA) and transmit-array (TA) antennas. We show that the precoders for RA and TA antennas have to meet different constraints compared to those for conventional MIMO architectures. Taking these constraints into account and exploiting the sparsity of mmWave channels, we design an efficient precoder for RA and TA antennas based on the orthogonal matching pursuit algorithm. Furthermore, in order to fairly compare the performance of RA and TA antennas with conventional fully-digital and hybrid MIMO architectures, we develop a unified power consumption model. Our simulation results show that unlike conventional MIMO architectures, RA and TA antennas are highly energy efficient and fully scalable in terms of the number of transmit antennas.

==> Fig/EE_M/EE_M.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{015}[cl][cl]{\matlabtextA TA OMP (Prop.)}%
\psfrag{016}[cl][cl]{\matlabtextA RA OMP (Prop.)}%
\psfrag{017}[cl][cl]{\matlabtextA RA AO \BB}%
\psfrag{018}[cl][cl]{\matlabtextA PC OMP (Prop.)}%
\psfrag{019}[cl][cl]{\matlabtextA FC OMP \CC}%
\psfrag{020}[cl][cl]{\matlabtextA FD SVD}%
\psfrag{021}[cl][cl]{\matlabtextA FI}%
\psfrag{022}[cl][cl]{\matlabtextA PI}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{15}{15}\selectfont\strut}%
\psfrag{023}[bc][bc]{\matlabtextB c)}%
\psfrag{024}[bc][bc]{\matlabtextB Energy Efficiency (MBits/Joule)}%
\psfrag{025}[tc][tc]{\matlabtextB Number of Antennas $M$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $200$}%
\psfrag{002}[ct][ct]{\matlabtextC $400$}%
\psfrag{003}[ct][ct]{\matlabtextC $600$}%
\psfrag{004}[ct][ct]{\matlabtextC $800$}%
\psfrag{005}[ct][ct]{\matlabtextC $1000$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $0$}%
\psfrag{007}[rc][rc]{\matlabtextC $50$}%
\psfrag{008}[rc][rc]{\matlabtextC $100$}%
\psfrag{009}[rc][rc]{\matlabtextC $150$}%
\psfrag{010}[rc][rc]{\matlabtextC $200$}%
\psfrag{011}[rc][rc]{\matlabtextC $250$}%
\psfrag{012}[rc][rc]{\matlabtextC $300$}%
\psfrag{013}[rc][rc]{\matlabtextC $350$}%
\psfrag{014}[rc][rc]{\matlabtextC $400$}%
%
%% </ytick>

==> Fig/PowerM/PowerM.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextA TA OMP (Prop.)}%
\psfrag{020}[cl][cl]{\matlabtextA RA OMP (Prop.)}%
\psfrag{021}[cl][cl]{\matlabtextA RA AO \BB}%
\psfrag{022}[cl][cl]{\matlabtextA PC OMP (Prop.)}%
\psfrag{023}[cl][cl]{\matlabtextA FC OMP \CC}%
\psfrag{024}[cl][cl]{\matlabtextA FD SVD}%
\psfrag{025}[cl][cl]{\matlabtextA FI}%
\psfrag{026}[cl][cl]{\matlabtextA PI}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{15}{15}\selectfont\strut}%
\psfrag{027}[bc][bc]{\matlabtextB b)}%
\psfrag{028}[bc][bc]{\matlabtextB Total Power Consumption (Watt)}%
\psfrag{029}[tc][tc]{\matlabtextB Number of Antennas $M$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $600$}%
\psfrag{001}[ct][ct]{\matlabtextC $700$}%
\psfrag{002}[ct][ct]{\matlabtextC $800$}%
%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{005}[ct][ct]{\matlabtextD $0$}%
\psfrag{006}[ct][ct]{\matlabtextD $200$}%
\psfrag{007}[ct][ct]{\matlabtextD $400$}%
\psfrag{008}[ct][ct]{\matlabtextD $600$}%
\psfrag{009}[ct][ct]{\matlabtextD $800$}%
\psfrag{010}[ct][ct]{\matlabtextD $1000$}%
%
%% </xtick>
%
%% <ytick>
%
\providecommand\matlabtextE{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{003}[rc][rc]{\matlabtextE $10$}%
\psfrag{004}[rc][rc]{\matlabtextE $15$}%
%
\providecommand\matlabtextF{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[rc][rc]{\matlabtextF $0$}%
\psfrag{012}[rc][rc]{\matlabtextF $50$}%
\psfrag{013}[rc][rc]{\matlabtextF $100$}%
\psfrag{014}[rc][rc]{\matlabtextF $150$}%
\psfrag{015}[rc][rc]{\matlabtextF $200$}%
\psfrag{016}[rc][rc]{\matlabtextF $250$}%
\psfrag{017}[rc][rc]{\matlabtextF $300$}%
\psfrag{018}[rc][rc]{\matlabtextF $350$}%
%
%% </ytick>

==> Fig/RateM/RateM.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{015}[cl][cl]{\matlabtextA TA OMP (Prop.)}%
\psfrag{016}[cl][cl]{\matlabtextA RA OMP (Prop.)}%
\psfrag{017}[cl][cl]{\matlabtextA RA AO \BB}%
\psfrag{018}[cl][cl]{\matlabtextA PC OMP (Prop.)}%
\psfrag{019}[cl][cl]{\matlabtextA FC OMP \CC}%
\psfrag{020}[cl][cl]{\matlabtextA FD SVD}%
\psfrag{021}[cl][cl]{\matlabtextA FI}%
\psfrag{022}[cl][cl]{\matlabtextA PI}%
\psfrag{023}[cl][cl]{\matlabtextA $M=1024$}%
\psfrag{024}[cl][cl]{\matlabtextA $M=256$}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{15}{15}\selectfont\strut}%
\psfrag{025}[bc][bc]{\matlabtextB a)}%
\psfrag{026}[bc][bc]{\matlabtextB Spectral Efficiency (Bits/s/Hz)}%
\psfrag{027}[tc][tc]{\matlabtextB Number of Antennas $M$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $200$}%
\psfrag{002}[ct][ct]{\matlabtextC $400$}%
\psfrag{003}[ct][ct]{\matlabtextC $600$}%
\psfrag{004}[ct][ct]{\matlabtextC $800$}%
\psfrag{005}[ct][ct]{\matlabtextC $1000$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $15$}%
\psfrag{007}[rc][rc]{\matlabtextC $20$}%
\psfrag{008}[rc][rc]{\matlabtextC $25$}%
\psfrag{009}[rc][rc]{\matlabtextC $30$}%
\psfrag{010}[rc][rc]{\matlabtextC $35$}%
\psfrag{011}[rc][rc]{\matlabtextC $40$}%
\psfrag{012}[rc][rc]{\matlabtextC $45$}%
\psfrag{013}[rc][rc]{\matlabtextC $50$}%
\psfrag{014}[rc][rc]{\matlabtextC $55$}%
%
%% </ytick>
